Optimizing Local Satisfaction of Long-Run Average Objectives in Markov Decision Processes

Long-run average optimization problems for Markov decision processes (MDPs) require constructing policies with optimal steady-state behavior, i.e., optimal limit frequency of visits to the states. However, such policies may suffer from local instability, i.e., the frequency of states visited in a bounded time horizon along a run differs significantly from the limit frequency. In this work, we propose an efficient algorithmic solution to this problem.

==> sections/figureone.tex <==
\begin{figure*}
    \includegraphics*[width=.55\textwidth]{big_comparison.pdf}
    \includegraphics*[width=.45\textwidth]{l-badness_at_5_a_memory=3.pdf}
    \caption{Strategies constructed for the graph of Fig.~\ref{fig-RM-system}. Adding more memory to the state $R$ helps. Best results are achieved for certain combinations of $\beta$ and $\gamma$ where $\beta+\gamma$ does not exceed the threshold around $0.6$.}
    \label{fig-exp-I}
\end{figure*}
    
